LLMs as On-demand Customizable Service

Large Language Models (LLMs) have demonstrated remarkable language understanding and generation capabilities. However, training, deploying, and accessing these models pose notable challenges, including resource-intensive demands, extended training durations, and scalability issues. To address these issues, we introduce a concept of hierarchical, distributed LLM architecture that aims at enhancing the accessibility and deployability of LLMs across heterogeneous computing platforms, including general-purpose computers (e.g., laptops) and IoT-style devices (e.g., embedded systems). By introducing a "layered" approach, the proposed architecture enables on-demand accessibility to LLMs as a customizable service. This approach also ensures optimal trade-offs between the available computational resources and the user's application needs. We envision that the concept of hierarchical LLM will empower extensive, crowd-sourced user bases to harness the capabilities of LLMs, thereby fostering advancements in AI technology in general.

==> Sections/attacks_on_FL.tex <==

%\section{Attacks on FL:}Federated Learning (FL) is vulnerable to various forms of attacks, including data poisoning attacks~\cite{datapoisoning} where participants intentionally submit data with incorrect labels, model poisoning attacks~\cite{modelpoisoning1,modelpoisoning2,modelpoisoning3} where malicious participants modify the updated model directly before sending it for aggregation, data modification attacks, free-riding attacks~\cite{freeriding} where malicious participants contribute passively, generative adversarial network (GAN) based attacks~\cite{gan1,gan2,gan3} that exploit training and poisoning data, membership inference attack (MIA)~\cite{mia1}, malicious server \etc

%Researchers propose diverse defense mechanisms in Federated Learning (FL) to address attacks. A sniper-based approach~\cite{sniper} identifies legitimate users and mitigates poisoning attacks. Analytic-based methods, including Auror~\cite{auror} and the Krum model~\cite{euclid1}, detect data and model poisoning through clustering and Euclidean distance, respectively. Autoencoders in multiple studies~\cite{auto1,auto2,auto3} identify malicious local models.  LFR (loss function-based rejection) and ERR (error rate-based rejection) techniques are proposed in~\cite{auto1}. The Foolsgold approach~\cite{foolsgold} combats Sybil-based, label flipping, and backdoor poisoning attacks. PDGAN~\cite{pdgan} defends against data poisoning by malicious clients. Additionally, secure multiparty computation (SMC) and differential privacy (DP) ensure secure FL models with high accuracy.  Trusted Execution Environments (TEEs) are defined as high-level trusted environments for executing code~\cite{whtaistee,trustedsurvey}, and they can be utilized to defend against malicious servers and protect training and inference data of the different nodes of federated architecture~\cite{tee1,tee2}. 




%Federated Learning (FL) is vulnerable to various forms of attacks, including data poisoning attacks~\cite{datapoisoning} where participants intentionally submit data with incorrect labels, model poisoning attacks~\cite{modelpoisoning1,modelpoisoning2,modelpoisoning3} where malicious participants modify the updated model directly before sending it for aggregation, data modification attacks, free-riding attacks~\cite{freeriding} where malicious participants contribute passively, generative adversarial network (GAN) based attacks~\cite{gan1,gan2,gan3} that exploit training and poisoning data, membership inference attack (MIA)~\cite{mia1}, malicious server \etc Researchers propose diverse defense mechanisms in Federated Learning (FL) to address attacks. A sniper-based approach~\cite{sniper} identifies legitimate users and mitigates poisoning attacks. Analytic-based methods, including Auror~\cite{auror} and the Krum model~\cite{euclid1}, detect data and model poisoning through clustering and Euclidean distance, respectively. Autoencoders in multiple studies~\cite{auto1,auto2,auto3} identify malicious local models.  LFR (loss function-based rejection) and ERR (error rate-based rejection) techniques are proposed in~\cite{auto1}. The Foolsgold approach~\cite{foolsgold} combats Sybil-based, label flipping, and backdoor poisoning attacks. PDGAN~\cite{pdgan} defends against data poisoning by malicious clients. Additionally, secure multiparty computation (SMC) and differential privacy (DP) ensure secure FL models with high accuracy.  Trusted Execution Environments (TEEs) are defined as high-level trusted environments for executing code~\cite{whtaistee,trustedsurvey}, and they can be utilized to defend against malicious servers and protect training and inference data of the different nodes of federated architecture~\cite{tee1,tee2}. 



%Researchers propose various defence mechanisms to address attacks in Federated Learning (FL). A sniper based approach~\cite{sniper} is suggested to identify legitimate users and reduce poisoning attack success. Analytic-based methods, such as Auror~\cite{auror} and the Krum model~\cite{euclid1}, detect data and model poisoning through clustering and Euclidean distance, respectively. Autoencoders are used in multiple works~\cite{auto1,auto2,auto3} to identify malicious local models. LFR and ERR techniques are proposed in reference 105. The Foolsgold approach~\cite{foolsgold} combats Sybil-based, label flipping, and backdoor poisoning attacks. PDGAN~\cite{pdgan}, a GAN-based method, defends against data poisoning from malicious FL clients. Additionally, secure multiparty computation (SMC) and differential privacy (DP) ensure secure FL models with high accuracy. Trusted Execution Environments (TEEs) safeguard against malicious servers and protect training and inference data~\cite{whtaistee,trustedsurvey}.The authors in~\cite{tee1,tee2} propose a framework that uses TEE in the federated environment.


%%Researchers have put forth a range of defense mechanisms to address these attacks. In one study (136), the authors propose a sniper approach that identifies legitimate users, thereby reducing the success rate of poisoning attacks. Analytic-based approaches have also been suggested by different authors to detect data poisoning and model poisoning attacks. For example, in reference [139], the authors propose Auror, a defense mechanism that performs clustering on each client update before the aggregation step to counter malicious client updates. In references [138, 147], the Krum model utilizes Euclidean distance to detect deviations in input parameters from each client. Autoencoders have been proposed in multiple works ([105, 148, 149, 150, 151]) as a means to identify malicious local models. In reference [105], the authors propose LFR (loss function-based rejection) and ERR (error rate-based rejection) techniques. Another approach, called Foolsgold, proposed in reference [145], is effective against Sybil-based, label flipping, and backdoor poisoning attacks. PDGAN, a GAN-based method introduced in [165], aims to defend against data poisoning attacks from malicious clients in FL.In addition to these techniques, secure multiparty computation (SMC) and differential privacy (DP) are employed to achieve a secure FL model with high accuracy. Trusted Execution Environments (TEEs) are defined as high-level trusted environments for executing code, and they can be utilized to defend against malicious servers and protect training and inference data.
